Hierarchical Clustering via Sketches and Hierarchical Correlation Clustering

Recently, Hierarchical Clustering (HC) has been considered through the lens of optimization. In particular, two maximization objectives have been defined. Moseley and Wang defined the \emph{Revenue} objective to handle similarity information given by a weighted graph on the data points (w.l.o.g., $[0,1]$ weights), while Cohen-Addad et al. defined the \emph{Dissimilarity} objective to handle dissimilarity information. In this paper, we prove structural lemmas for both objectives allowing us to convert any HC tree to a tree with constant number of internal nodes while incurring an arbitrarily small loss in each objective. Although the best-known approximations are 0.585 and 0.667 respectively, using our lemmas we obtain approximations arbitrarily close to 1, if not all weights are small (i.e., there exist constants $\epsilon, \delta$ such that the fraction of weights smaller than $\delta$, is at most $1 - \epsilon$); such instances encompass many metric-based similarity instances, thereby improving upon prior work. Finally, we introduce Hierarchical Correlation Clustering (HCC) to handle instances that contain similarity and dissimilarity information simultaneously. For HCC, we provide an approximation of 0.4767 and for complementary similarity/dissimilarity weights (analogous to $+/-$ correlation clustering), we again present nearly-optimal approximations.

==> reduction_to_metrics.tex <==
\section{Reduction to Metrics}

Let $g$ define a non-increasing function $g \in \mathcal{R} \rightarrow [0,1]$. Given two data points $i$ and $j$ let $d_{ij}$ denote their distance as defined by our metric. Let $M$ denote the doubling dimension of our metric. Define $A = A(\epsilon)$ to be the tree generated by the algorithm that adds $\epsilon$ to all weights and then runs our PTAS for dense graphs. We note that $A$ is well defined since the altered weights define a dense graph for any constant $\epsilon$.

\begin{proof}
Let $w_{ij} = g(d_{ij})$ and let $w'_{ij} = w_{ij} + \epsilon$. Denote by $O$ and $O'$ the trees which generate the maximal revenue with respect to $w_{ij}$ and $w'_{ij}$ respectively. Finally, given an HC tree, let $Rev(T)$ and $Rev'(T)$ denote the revenue generated by $T$ with respect to $w_{ij}$ and $w'_{ij}$ respectively. Therefore, for any constant $\delta$ we have that,
\begin{align*}
Rev'(A) \geq (1 - \delta)Rev'(O') \geq (1 - \delta)Rev'(O).
\end{align*}

Note that for any tree $T$, $\sum_{ij}(n - T_{ij}) = \frac{n^3}{6} - \frac{n^2}{2} + \frac{n}{3}$ (since this is the revenue generated in a clique instance). By the definition of $w'_{ij}$, we get,
\begin{align*}
Rev(A) \geq (1 - \delta)Rev(O) - \delta \epsilon \frac{n^3}{6}.
\end{align*}

Let $\alpha$ denote our metric diameter. Since our metric has doubling dimension $M$ there are $M^2$ balls of radius $\alpha/4$ that cover all our data points. Therefore, there are at most ${M^2 choose 2}(\frac{n}{M^2})^2 = n^2(\frac{1}{2} - \frac{1}{2M^2})$ pairs of distance $\geq \alpha/2$. Therefore,
\begin{align*}
W = \sum_{i,j}w_{ij} = \sum g(d_{ij}) \geq \frac{n^2}{2M^2}g(\alpha/2).
\end{align*}

\noindent Since $Rev(O) \geq \frac{n}{3}W$, we are guaranteed that $\frac{M^2}{g(\alpha/2)}\cdot Rev(O) \geq \frac{n^3}{6}$. Therefore,
\begin{align*}
Rev(A) \geq (1 - \delta -\delta \epsilon \frac{M^2}{g(\alpha/2)})Rev(O).
\end{align*}

\noindent Thus, if $M$ and $g(\alpha/2)$ are constant, our algorithm yields a PTAS.
\end{proof}
